A 2-3 mm high-resolution molecular line survey towards the centre of the nearby spiral galaxy NGC 6946

The complex physical, kinematic, and chemical properties of galaxy centres make them interesting environments to examine with molecular line emission. We present new $2-4$" (${\sim}75{-}150$ pc at $7.7$ Mpc) observations at 2 and 3 mm covering the central $50$" (${\sim}1.9$ kpc) of the nearby double-barred spiral galaxy NGC 6946 obtained with the IRAM Plateau de Bure Interferometer. We detect spectral lines from ten molecules: CO, HCN, HCO$^+$, HNC, CS, HC$_3$N, N$_2$H$^+$, C$_2$H, CH$_3$OH, and H$_2$CO. We complemented these with published 1mm CO observations and 33 GHz continuum observations to explore the star formation rate surface density ${\Sigma_{\mathrm{SFR}}}$ on 150 pc scales. In this paper, we analyse regions associated with the inner bar of NGC 6946 $-$ the nuclear region (NUC), the northern (NBE), and southern inner bar end (SBE) and we focus on short-spacing corrected bulk (CO) and dense gas tracers (HCN, HCO$^+$, and HNC). We find that HCO$^+$ correlates best with ${\Sigma_{\mathrm{SFR}}}$, but the dense gas fraction ($f_{\mathrm{dense}}$) and star formation efficiency of the dense gas (${\mathrm{SFE_{dense}}}$) fits show different behaviours than expected from large-scale disc observations.The SBE has a higher ${\Sigma_{\mathrm{SFR}}}$, $f_{\mathrm{dense}}$, and shocked gas fraction than the NBE. We examine line ratio diagnostics and find a higher CO(2-1)/CO(1-0) ratio towards NBE than for the NUC. Moreover, comparison with existing extragalactic datasets suggests that using the HCN/HNC ratio to probe kinetic temperatures is not suitable on kiloparsec and sub-kiloparsec scales in extragalactic regions. Lastly, our study shows that the HCO$^+$/HCN ratio might not be a unique indicator to diagnose AGN activity in galaxies.

==> Figures/01caption/figure1.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/plots/gallary_v4_compressed-1.pdf}
    \caption{\textbf{Gallery of the multi-wavelength observation towards the centre of NGC\,6946 }
    {\em Left panels:} (a) three colour optical image, with the region of interest drawn as a purple box, (b) CO\,(1-0) emission shown in contours levels of 60, 90, 200, 300, 600, and are repeated on all panels for comparison, (c) integrated CO\,(1-0) emission shown in colour scale, (d) CO\,(2-1) emission towards the inner $20\arcsec$ shown as colour scale; {\em Sketch (right):} denoting all observed features (see Section~\ref{sec:story-about-central-region} for an overview), {\bf Panels on next page:} (e)--(g) continuum emission, (h)--(j) infrared emission and (k)--(m) hydrogen recombination lines and $X$-ray emission (see Table~\ref{tab:fig1-ref} for references of all observations shown). The rightmost column shows integrated intensity maps of three of our fourteen detected emission lines for comparison. Optical image credits: NASA, ESA, STScI, R.~Gendler, and the Subaru Telescope (NAOJ).}
    \label{fig:color}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/plots/gallary_v4_compressed-2.pdf}
    \contcaption{}
    \label{}
\end{figure*}



==> Figures/01caption/figure3_referee_format.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/plots/spectra_v3.pdf}
    \caption{\textbf{Spectra of fourteen emission lines:} We show the spectra of all the emission lines detected within this survey for the central sight line, i.e. aperture of $4\arcsec \approx 150$~pc. The pink dotted rectangle shows the ones we use for discussing line ratio diagnostic plots later in this work (Section~\ref{sec:Discussion}). We normalise all of them to the maximum value in their spectra. The right-hand side indicates what each molecule could be tracing according to literature. Within each group we ordered the spectra by their \SN.} 
    %is mainly tracing in our context.} 
    \label{fig:central-sightline-spectra}
\end{figure}

==> Figures/01caption/figure5_referee_format.tex <==
\begin{figure}[ht!]
\centering
    \includegraphics[width=0.5 \linewidth]{Figures/plots/RatioMaps_v2.pdf}
    \caption{\textbf{Line ratio maps of the central $\bm{20\arcsec}$.} We show the line ratio maps for the central $20\arcsec \approx 750$~pc. We overplot on each map contours of the \chem{CO}{21} integrated intensity map in red and denote the features associated with the inner bar (see Figure~\ref{fig:SFR-and-mask} for the region mask).}
    \label{fig:RatioMaps-uvtrimmed-SSC}
\end{figure}

==> Figures/01caption/figure6_referee_format.tex <==
\begin{figure*}[ht!]
    \includegraphics[width=1.0\linewidth]{Figures/plots/Correlations1-3_v4.pdf}
    \caption{\textbf{Correlation plots ordered by their slope, $\beta$.} Dark purple colours show HCN, purple HCO$^+$ and pink HNC. \textit{Top row}: Integrated intensities of the dense gas tracers (ordered by their slope, $\beta$) versus \sigsfr. \textit{Middle row}: Integrated intensity of \chem{CO}{21} -- an indicator of the mean volume density -- versus the line ratio with \chem{CO}{21} -- a~spectroscopic tracers of \fdense\ ;  \textit{Bottom row:} Integrated intensity of \chem{CO}{21} -- an indicator of the mean volume density -- versus the ratio of \sigsfr\ with the dense gas tracers -- a~spectroscopic tracers of \sfedense. The \texttt{linmix} fits (accounting for upper limits) are shown as solid lines surrounded by $3\sigma$ confidence intervals (shaded regions of corresponding colours). Absolute uncertainties are plotted on each data point, which are generally small towards the regions NUC, NBE and SBE. We find the highest uncertainties in the outskirts in our \sigsfr\ map. Correlations including HNC result in 58 significant sight lines and 15 upper limits (denoted as light pink markers). We display in each panel Pearson's correlation coefficient and the power-law slope, intercept and $p$-value (see Table~\ref{tab:Corr}).}
    \label{fig:Corr}
\end{figure*}

==> Figures/01caption/figure7_referee_format.tex <==
\begin{figure}[ht!]
\centering
    \includegraphics[width=0.5 \linewidth]{Figures/plots/R21.pdf}
    \caption{ \textbf{$\bm{R_{21}}$ against galactocentric radius.} The circular shaped markers represent all of the $R_{21}$ values for the central $20\arcsec\approx745$~pc coloured by their \fdense. The different sizes show their varying signal-to-noise ratio in \cotwo. Additionally, we overplot the contours of the three different regions: The cyan color refers to the nuclear region (NUC), the green to the northern bar end (NBE) and the magenta to the southern bar end (SBE). Along the galactocentric radius, we find in the centre higher $R_{21}$ values, an initial steady decrease followed by a gradual increase. $R_{21}$ towards NBE is higher than expected (more in Section~\ref{sec:R21}).}
    \label{fig:R21}
\end{figure}

==> Figures/01caption/figure9_referee_format.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5 \linewidth]{Figures/plots/LRP-v3.pdf}
    \caption{\textbf{Line ratios for the nuclear region and inner-bar ends:} \textit{Top}: Scatter plot showing the mean line ratios of the 7~hexagonal points for each molecule on the $y$-axis with respect to \chem{CO}{21}. For visualisation purpose we spaced the markers along the $x$-axis. The different shapes of the markers present the defined regions.  The colorbar shows the normalised \chem{CO}{21} integrated intensity to the mean \chem{CO}{21} value.  
    We plot the propagated errors in grey and find that they are very small. For the ratios we applied a signal-to-noise cut (see Section~\ref{Sec:Res-LineRatios}). \textit{Bottom}: The relative differences of the line ratios with respect to the mean of the line ratios among the different regions (linear-scale).}
    \label{fig:regions}
\end{figure}

